The Cost of Learning: Efficiency vs. Efficacy of Learning-Based RRM for 6G

In the past few years, Deep Reinforcement Learning (DRL) has become a valuable solution to automatically learn efficient resource management strategies in complex networks. In many scenarios, the learning task is performed in the Cloud, while experience samples are generated directly by edge nodes or users. Therefore, the learning task involves some data exchange which, in turn, subtracts a certain amount of transmission resources from the system. This creates a friction between the need to speed up convergence towards an effective strategy, which requires the allocation of resources to transmit learning samples, and the need to maximize the amount of resources used for data plane communication, maximizing users' Quality of Service (QoS), which requires the learning process to be efficient, i.e., minimize its overhead. In this paper, we investigate this trade-off and propose a dynamic balancing strategy between the learning and data planes, which allows the centralized learning agent to quickly converge to an efficient resource allocation strategy while minimizing the impact on QoS. Simulation results show that the proposed method outperforms static allocation methods, converging to the optimal policy (i.e., maximum efficacy and minimum overhead of the learning plane) in the long run.

==> biblio.tex <==
@inproceedings{mason2022no,
  title={No Free Lunch: Balancing Learning and Exploitation at the Network Edge},
  author={Mason, Federico and Chiariotti, Federico and Zanella, Andrea},
  booktitle={International Conference on Communications (ICC)},
  pages={631--636},
  year={2022},
  organization={IEEE}
}

@article{chih2021ai,
  title={{AI} as an Essential Element of a {Green 6G}},
  author={Chih-Lin, I},
  journal={IEEE Transactions on Green Communications and Networking},
  volume={5},
  number={1},
  pages={1--3},
  year={2021},
  publisher={IEEE}
}

@article{chen2019deep,
  title={Deep Learning With Edge Computing: A Review.},
  author={Chen, Jiasi and Ran, Xukan},
  journal={Proceedings of the IEEE},
  volume={107},
  number={8},
  pages={1655--1674},
  year={2019}
}

@article{khan2020federated,
  title={Federated learning for edge networks: Resource optimization and incentive mechanism},
  author={Khan, Latif U and Pandey, Shashi Raj and Tran, Nguyen H and Saad, Walid and Han, Zhu and Nguyen, Minh NH and Hong, Choong Seon},
  journal={IEEE Communications Magazine},
  volume={58},
  number={10},
  pages={88--93},
  year={2020},
  publisher={IEEE}
}

@inproceedings{villacca2021online,
  title={Online Learning under Resource Constraints},
  author={Villa{\c{c}}a, Rodolfo S and Stadler, Rolf},
  booktitle={International Symposium on Integrated Network Management (IM)},
  pages={134--142},
  year={2021},
  organization={IFIP/IEEE}
}

@inproceedings{luo2021cost,
  title={Cost-effective federated learning design},
  author={Luo, Bing and Li, Xiang and Wang, Shiqiang and Huang, Jianwei and Tassiulas, Leandros},
  booktitle={Conference on Computer Communications (INFOCOM)},
  year={2021},
  organization={IEEE}
}

@inproceedings{chan2018learning,
  title={Learning network architectures of deep {CNNs} under resource constraints},
  author={Chan, Michael and Scarafoni, Daniel and Duarte, Ronald and Thornton, Jason and Skelly, Luke},
  booktitle={Conference on Computer Vision and Pattern Recognition (CVPR) Workshops},
  pages={1703--1710},
  organization={IEEE},
  year={2018}
}

@article{beaumont2021efficient,
  title={Efficient Combination of Rematerialization and Offloading for Training {DNNs}},
  author={Beaumont, Olivier and Eyraud-Dubois, Lionel and Shilova, Alena},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={23844--23857},
  year={2021}
}

@article{mnih2015human,
  title={Human-level control through deep reinforcement learning},
  author={Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Rusu, Andrei A and Veness, Joel and Bellemare, Marc G and Graves, Alex and Riedmiller, Martin and Fidjeland, Andreas K and Ostrovski, Georg and others},
  journal={Nature},
  volume={518},
  number={7540},
  pages={529--533},
  year={2015},
  publisher={Nature Publishing Group}
}


@article{jang2020knowledge,
  title={Knowledge Transfer for On-Device Deep Reinforcement Learning in Resource Constrained Edge Computing Systems},
  author={Jang, Ingook and Kim, Hyunseok and Lee, Donghun and Son, Young-Sung and Kim, Seonghyun},
  journal={IEEE Access},
  volume={8},
  pages={146588--146597},
  year={2020},
  publisher={IEEE}
}

@article{patterson2021carbon,
  title={Carbon emissions and large neural network training},
  author={Patterson, David and Gonzalez, Joseph and Le, Quoc and Liang, Chen and Munguia, Lluis-Miquel and Rothchild, Daniel and So, David and Texier, Maud and Dean, Jeff},
  journal={arXiv preprint arXiv:2104.10350},
  year={2021}
}


@book{sutton2018reinforcement,
  title={Reinforcement learning: An introduction},
  author={Sutton, Richard S and Barto, Andrew G},
  year={2018},
  publisher={MIT press}
}


@article{sami2021ai,
  title={{AI}-based resource provisioning of {IoE} services in {6G}: A deep reinforcement learning approach},
  author={Sami, Hani and Otrok, Hadi and Bentahar, Jamal and Mourad, Azzam},
  journal={IEEE Transactions on Network and Service Management},
  volume={18},
  number={3},
  pages={3527--3540},
  year={2021},
  publisher={IEEE}
}


@article{letaief2019roadmap,
  title={The roadmap to {6G: AI} empowered wireless networks},
  author={Letaief, Khaled B and Chen, Wei and Shi, Yuanming and Zhang, Jun and Zhang, Ying-Jun Angela},
  journal={IEEE Communications Magazine},
  volume={57},
  number={8},
  pages={84--90},
  year={2019},
  publisher={IEEE}
}


@article{hu2021energy,
  title={An energy-efficient in-network computing paradigm for {6G}},
  author={Hu, Ning and Tian, Zhihong and Du, Xiaojiang and Guizani, Mohsen},
  journal={IEEE Transactions on Green Communications and Networking},
  volume={5},
  number={4},
  pages={1722--1733},
  year={2021},
  publisher={IEEE}
}


@ARTICLE{rlInNetworkingSurvey,
  author={Luong, Nguyen Cong and Hoang, Dinh Thai and Gong, Shimin and Niyato, Dusit and Wang, Ping and Liang, Ying-Chang and Kim, Dong In},
  journal={IEEE Communications Surveys \& Tutorials}, 
  title={Applications of Deep Reinforcement Learning in Communications and Networking: A Survey}, 
  year={2019},
  volume={21},
  number={4},
  pages={3133-3174},
  doi={10.1109/COMST.2019.2916583}}

@misc{neda2022survey,
  doi = {10.48550/ARXIV.2209.14141},
  url = {https://arxiv.org/abs/2209.14141},
  author = {Shalavi, Neda and Perin, Giovanni and Zanella, Andrea and Rossi, Michele},
  keywords = {Networking and Internet Architecture (cs.NI), Distributed, Parallel, and Cluster Computing (cs.DC), FOS: Computer and information sciences, FOS: Computer and information sciences, C.2},
  title = {Energy Efficient Deployment and Orchestration of Computing Resources at the Network Edge: a Survey on Algorithms, Trends and Open Challenges},
  publisher = {arXiv},
  year = {2022},
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{pqk_survey,
title = {Pruning and quantization for deep neural network acceleration: A survey},
journal = {Neurocomputing},
volume = {461},
pages = {370-403},
year = {2021},
issn = {0925-2312},
doi = {https://doi.org/10.1016/j.neucom.2021.07.045},
url = {https://www.sciencedirect.com/science/article/pii/S0925231221010894},
author = {Tailin Liang and John Glossner and Lei Wang and Shaobo Shi and Xiaotong Zhang},
keywords = {Convolutional neural network, Neural network acceleration, Neural network quantization, Neural network pruning, Low-bit mathematics},
}
